Metrics reloaded: Recommendations for image analysis validation

Increasing evidence shows that flaws in machine learning (ML) algorithm validation are an underestimated global problem. Particularly in automatic biomedical image analysis, chosen performance metrics often do not reflect the domain interest, thus failing to adequately measure scientific progress and hindering translation of ML techniques into practice. To overcome this, our large international expert consortium created Metrics Reloaded, a comprehensive framework guiding researchers in the problem-aware selection of metrics. Following the convergence of ML methodology across application domains, Metrics Reloaded fosters the convergence of validation methodology. The framework was developed in a multi-stage Delphi process and is based on the novel concept of a problem fingerprint - a structured representation of the given problem that captures all aspects that are relevant for metric selection, from the domain interest to the properties of the target structure(s), data set and algorithm output. Based on the problem fingerprint, users are guided through the process of choosing and applying appropriate validation metrics while being made aware of potential pitfalls. Metrics Reloaded targets image analysis problems that can be interpreted as a classification task at image, object or pixel level, namely image-level classification, object detection, semantic segmentation, and instance segmentation tasks. To improve the user experience, we implemented the framework in the Metrics Reloaded online tool, which also provides a point of access to explore weaknesses, strengths and specific recommendations for the most common validation metrics. The broad applicability of our framework across domains is demonstrated by an instantiation for various biological and medical image analysis use cases.

==> Author-contributions.tex <==
\section*{Author contributions}
L.M.-H. initiated and led the study, was a member of the Delphi core team, wrote and reviewed the manuscript, prepared and evaluated all surveys, organized all workshops, tested the online toolkit, and organized the social media campaign.
A.R. initiated and led the study, was a member of the Delphi core team, wrote and reviewed the manuscript, prepared and evaluated all surveys, organized all workshops, tested the metric mappings and the online toolkit, organized the social media campaign, and designed all figures.
P.F.J. initiated and led the study, was a member of the Delphi core team, led the \ac{ObD} and \ac{InS} expert group, wrote and reviewed the manuscript, prepared and evaluated all surveys, organized all workshops, tested the metric mappings and the online toolkit, organized the social media campaign, and participated in surveys.
P.G. led the \ac{ImLC} expert group, was a member of the extended Delphi core team, wrote and reviewed the manuscript, prepared the BPMN diagrams, tested the online toolkit, and participated in surveys and workshops.
M.D.T. was a member of the extended Delphi core team and wrote and reviewed the manuscript.
F.B. led the calibration expert group, reviewed the manuscript, and participated in surveys.
E.C. led the cross topic expert group, was a member of the extended Delphi core team, and reviewed the manuscript.
B.G. led the cross-topic expert group and was an active member of the \ac{SemS} expert group, reviewed the manuscript, and participated in surveys and workshops.
F.I. led the \ac{SemS} expert group, reviewed the manuscript, tested the online toolkit, and participated in surveys and workshops.
J.K. led the biomedical expert group, reviewed the manuscript, and participated in surveys and workshops.
M.K. led the \ac{ObD} and \ac{InS} expert group, reviewed the manuscript, and participated in surveys and workshops.
M.R. led the \ac{SemS} expert group, reviewed the manuscript, and participated in surveys and workshops.
M.A.R. led the \ac{ImLC} expert group, reviewed the manuscript, tested the metric mappings, and participated in surveys and workshops.
M.W. co-led the cross-topic expert group.
A.E.K. implemented the online toolkit and was a member of the extended Delphi core team.
C.H.S. implemented the reference implementations of all metrics in Python, was an active member of the \ac{ObD} and \ac{InS} expert group, reviewed the manuscript, and participated in surveys workshops.
Mi.B. was a member of the extended Delphi core team, was an active member of the \ac{ObD} and \ac{InS} expert group, wrote and reviewed the manuscript, tested the metric mappings and the online toolkit, and participated in surveys and workshops.
M.E. was a member of the extended Delphi core team, prepared the BPMN diagrams, reviewed the document, assisted in survey preparation, tested the metric mappings and the online toolkit, and participated in surveys.
D.H.-N. was a member of the extended Delphi core team and prepared all surveys.
T.R. was a member of the extended Delphi core team, was an active member of the \ac{ObD} and \ac{InS} expert group, wrote and reviewed the document, assisted in survey preparation, tested the metric mappings and the online toolkit, and participated in surveys and workshops.
L.A. reviewed the manuscript and participated in surveys and workshops.
M.A. was an active member of the \ac{SemS} expert group and participated in surveys and workshops.
T.A. was an active member of the \ac{ObD} and \ac{InS} expert group, tested the metric mappings, reviewed the manuscript, and participated in surveys and workshops.
S.B. co-led the \ac{SemS} expert group, reviewed the manuscript, and participated in surveys and workshops.
A.B. was an active member of the biomedical and cross-topic expert groups, reviewed the manuscript, and participated in surveys and workshops.
M.B.B. triggered changes in the framework by responding to public questionnaire, reviewed the manuscript, and participated in surveys.
M.J.C. was an active member of the \ac{ImLC} expert group and participated in surveys and workshops.
V.C. was an active member of the \ac{ImLC} and cross-topic expert groups, reviewed the manuscript, and participated in surveys and workshops.
B.A.C. was an active member of the \ac{ObD} and \ac{InS} expert group, tested the metric mappings, reviewed the manuscript, and participated in surveys and workshops.
K.F. was an active member of the biomedical and cross-topic expert groups and participated in surveys and workshops.
L.F. triggered changes in the framework by responding to public questionnaire, was an active member of the calibration expert group, reviewed the manuscript, and participated in surveys.
A.G. triggered changes in the framework by responding to public questionnaire, was an active member of the calibration expert group, reviewed the manuscript, and participated in surveys.
B.v.G. participated in surveys and workshops.
R.H. triggered changes in the framework by responding to public questionnaire and participated in surveys.
D.A.H. was an active member of the biomedical and cross-topic expert groups, reviewed the manuscript, and participated in surveys and workshops.
M.M.H. was an active member of the \ac{ImLC} expert group, reviewed the manuscript, and participated in surveys and workshops.
M.H. co-led the biomedical expert group, was an active member of the cross-topic expert group, reviewed the manuscript, and participated in surveys and workshops.
P.J. co-led the cross-topic expert group, was an active member of the \ac{ObD} and \ac{InS} expert group, reviewed the manuscript, and participated in surveys and workshops.
C.E.K. was an active member of the biomedical expert group, reviewed the manuscript, and participated in surveys and workshops.
D.K. triggered changes in the framework by responding to public questionnaire and participated in surveys.
B.K. triggered changes in the framework by responding to public questionnaire, reviewed the manuscript, and participated in surveys.
F.K. triggered changes in the framework by responding to public questionnaire and participated in surveys.
A.K.-S. was a member of the extended Delphi core team and was an active member of the cross-topic group.
A.Kr. was an active member of the biomedical expert group, reviewed the manuscript, and participated in surveys and workshops.
B.A.L. was an active member of the \ac{SemS} expert group and participated in surveys and workshops.
G.L. was an active member of the \ac{ImLC} expert group, reviewed the manuscript, and participated in surveys and workshops.
A.M. was an active member of the biomedical and \ac{SemS} expert groups and participated in surveys and workshops.
K.M.-H. was an active member of the \ac{SemS} expert group, reviewed the manuscript, and participated in surveys and workshops.
E.M. was an active member of the \ac{ImLC} expert group, reviewed the manuscript, and participated in surveys.
B.M. participated in surveys and workshops.
K.G.M.M. was an active member of the cross-topic expert group, reviewed the manuscript, and participated in surveys and workshops.
H.M. was an active member of the \ac{ImLC} expert group, tested the metric mappings, reviewed the manuscript, and participated in surveys and workshops.
B.N. was an active member of the \ac{ObD} and \ac{InS} expert group, tested the metric mappings, reviewed the manuscript, and participated in surveys.
N.Ri. was an active member of the \ac{SemS} expert group and participated in surveys and workshops.
R.M.S. was an active member of the \ac{ObD} and \ac{InS}, the biomedical, and the cross-topic expert groups, reviewed the manuscript, and participated in surveys and workshops.
A.A.T. co-led the \ac{SemS} expert group and participated in surveys and workshops.
A.T. was an active member of the calibration group, reviewed the manuscript, and participated in surveys.
S.A.T. was an active member of the \ac{ObD} and \ac{InS} expert group, tested the metric mappings, reviewed the manuscript, and participated in surveys and workshops.
B.v.C. was an active member of the cross-topic expert group and participated in surveys.
G.V. was an active member of the \ac{ImLC} and cross-topic expert groups, reviewed the manuscript, and participated in surveys and workshops.
G.S.C., A.Kart., Ta.K., A.L.M., P.M., F.N., J.P., N.Ra., J.S.-R.,C.I.S., S.S., and M.v.S. served on the expert Delphi panel and participated in workshops and surveys.


==> Metric_Properties.tex <==
\vspace*{-\baselineskip}
{\tiny
\begin{table}[H]
\caption{\textbf{Properties of recommended reference-based metrics for image-level classification.} For all metrics, the considered cardinalities are provided along with the popularity, interpretability, and potential prevalence dependency. Several metrics allow for the definition of costs for class confusions (e.g. the penalization of \ac{FP} and \ac{FN} in the binary case), as indicated by the column \textit{allows individual confusion costs}. While many metrics focus on the Sensitivity and Specificity related to a class, other metrics also account for predictive values (\ac{PPV} and \ac{NPV}), as indicated by the column \textit{demands high predictive values}. Finally \textit{equal class weighing} indicates whether the metric assumes an equal weighing of classes. Abbreviations: \acf{BA}, \acf{EC}, \acf{MCC}, \acf{WCK}, \acf{LR+}, \acf{NB}, \acf{NPV}, \acf{PPV}, \acf{AP}, \acf{AUROC}.}
\label{tab:metric-properties}

\begin{tabular}{p{0.9cm}p{1.2cm}p{1.8cm}p{0.9cm}p{1.5cm}p{1.5cm}p{0.9cm}cccc}


\toprule
\textbf{Metric} & \textbf{Popularity} & \textbf{Interpretability} & \textbf{Prevalence dependency} & \textbf{Allows individual confusion costs} & \textbf{Demands high predictive values} & \textbf{Equal class weighing} & \multicolumn{4}{c}{\textbf{Cardinalities}}  \\
& & & & & & & \ac{TP} & \ac{FN} & \ac{FP} & \ac{TN}\\
\midrule
\multicolumn{11}{c}{\textbf{Multi-class Counting Metrics}} \\
\midrule

\rowcolor[HTML]{C0C0C0} 
Accuracy & very common & easy & yes & no & no & no & x & x & x & x \\
\rowcolor[HTML]{EFEFEF} 
\acs{BA} & common & easy & no & no & no & yes & x & x & x & x\\
\rowcolor[HTML]{C0C0C0}
\acs{EC} & uncommon & intuitive, \acs{ECN} variant allows for interpretable scaling & optional & yes & \acs{ECN} does, otherwise no & optional & x & x & x & x\\
\rowcolor[HTML]{EFEFEF} 
\acs{MCC} & uncommon & limited, minimum not pre-determined in multi-class & yes & no & yes & yes & x & x & x & x\\
\rowcolor[HTML]{C0C0C0} 
\acs{WCK} & Quadratic version common in ordinal scenarios  & limited, maximum value depends on prevalences & yes & yes & no & yes & x & x & x & x\\

\rowcolor[HTML]{FFFFFF}
\midrule
\multicolumn{11}{c}{\textbf{Per-class Counting Metrics}} \\
\midrule

\rowcolor[HTML]{C0C0C0} 
F$_\beta$ Score & very common & limited & yes  & limited since $\beta$ weighs confusions in relation to \acs{TP} & yes, for the positive class & no & x & x & x & \\
\rowcolor[HTML]{EFEFEF} 
\acs{LR+} & uncommon &  good for binary task & no & no & no & yes & x & x & x & x\\
\rowcolor[HTML]{C0C0C0} 
\acs{NB} & uncommon & limited & yes & limited, only \acs{FP} & no & no & x & x & x & x\\
\rowcolor[HTML]{EFEFEF} 
\acs{NPV}* & neutral & easy & yes & no & yes, for the negative class & no &  & x &  & x\\
\rowcolor[HTML]{C0C0C0} 
\acs{PPV}* & common & easy & yes & no & yes, for the positive class & no & x &  & x & \\
\rowcolor[HTML]{EFEFEF} 
Sensitivity* & common & easy & no & no & no & no & x & x &  & \\
\rowcolor[HTML]{C0C0C0} 
Specificity* & neutral & easy & no & no & no & no &  &  & x & x \\

\rowcolor[HTML]{FFFFFF}
\midrule
\multicolumn{11}{c}{\textbf{Multi-threshold Metrics}} \\
\midrule

\rowcolor[HTML]{C0C0C0} 
\acs{AP} & common & limited & yes & no & yes, for the positive class & no & x & x & x & \\
\rowcolor[HTML]{EFEFEF} 
\acs{AUROC} & very common & probabilistic interpretation is intuitive & no &  no & no & yes & x & x & x & x \\

\bottomrule
\multicolumn{11}{p{0.9\linewidth}}{ *: This metric might be used in combination with another metric using a predefined target value (see "Target value-based cutoff" in the definition of \textit{FP2.6: Cutoff on predicted class scores} (Suppl. Note~\ref{app:fingerprint-category}).} \\
\end{tabular}
\end{table}
\normalsize
}

==> Subprocesses.tex <==
%------------------------------------
%\input{Problem-Category-Mapping.tex}

%\newpage
%\subsection{Subprocesses used for %etric selection}
%\label{app:subprocesses-metric-selection}
%------------------------------------
%\acresetall

%An overview of the complete recommendation process is given in Fig.~\ref{fig:meta-mapping}. This sections provides the individual subprocesses referred to in the overview figure and indicated by the $\boxplus$-symbol. 


\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{images/MetricMappings/S1_category_mapping.pdf}
    %\includegraphics[width=1\linewidth]{images/MetricMappings/Delta/S1_category_mapping.pdf}
    \caption{\textbf{Subprocess S1 for selecting a problem category.} The \textit{Category Mapping} maps a given research problem to the appropriate problem category with the goal of \textbf{grouping problems by similarity of validation.} The leaf nodes represent the categories: image-level classification, object detection, instance segmentation, or semantic segmentation. FP2.1 refers to fingerprint 2.1 (see Fig.~\ref{fig:fingerprint-ss-1}). An overview of the symbols used in the process diagram is provided in Fig.~\ref{fig:process-diagram-symbols}.}
    \label{fig:category_mapping}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{images/MetricMappings/S2_subroutine_multi-class.pdf}
    %\includegraphics[width=1\linewidth]{images/MetricMappings/Delta/S2_subroutine_multi-class.pdf}
    \caption{\textbf{Subprocess S2 for selecting multi-class metrics (if any)}. Applies to: image-level classification (ImLC). In the case of presence of class imbalance and no compensation of class imbalance being requested, one should follow the "No" branch. Decision guides are provided in Suppl. Note~\ref{ssec:dg2}. A detailed description of the subprocess is given in Suppl. Note~\ref{app:ilc}.} 
    \label{fig:metric-selection:s2-multi-class}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{images/MetricMappings/S3_subroutine_single-threshold.pdf}
    % \includegraphics[width=1\linewidth]{images/MetricMappings/Delta/S3_subroutine_single-threshold.pdf}
    \caption{\textbf{Subprocess S3 for selecting a per-class counting metric (if any)}. Applies to: image-level classification (ImLC), object detection (ObD), and instance segmentation (InS). Decision guides are provided in Suppl. Note~\ref{ssec:dg3}. A detailed description of the subprocess is given in Suppl. Notes~\ref{app:ilc}, \ref{app:od} and \ref{app:is}.}
    \label{fig:metric-selection:s3-single-threshold}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{images/MetricMappings/S4_subroutine_multi-threshold.pdf}
     % \includegraphics[width=1\linewidth]{images/MetricMappings/Delta/S4_subroutine_multi-threshold.pdf}
    \caption{\textbf{Subprocess S4 for selecting a multi-threshold metric (if any)}. Applies to: image-level classification (ImLC), object detection (ObD), and instance segmentation (InS). Decision guides are provided in Suppl. Note~\ref{ssec:dg4}. A detailed description of the subprocess is given in Suppl. Notes~\ref{app:ilc}, \ref{app:od} and \ref{app:is}.}
    \label{fig:metric-selection:s4-multi-threshold}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{images/MetricMappings/S5_subroutine_calibration.pdf}
    % \includegraphics[width=1\linewidth]{images/MetricMappings/Delta/S5_subroutine_calibration.pdf}
    \caption{\textbf{Subprocess S5 for selecting a calibration metric (if any)}. Applies to: image-level classification (ImLC). Decision guides are provided in Suppl. Note~\ref{ssec:dg5}. A detailed description of the subprocess is given in Suppl. Note~\ref{app:calibration}. Further suggested calibration metrics include the calibration loss \cite{brummer2006application}, calibration slope \cite{steyerberg2010assessing}, \acf{ECI} \cite{van2015spline} and \acf{O:E ratio} \cite{riley2016external}.}
    \label{fig:metric-selection:s5-calibration}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{images/MetricMappings/S6_subroutine_overlap.pdf}
    % \includegraphics[width=1\linewidth]{images/MetricMappings/Delta/S6_subroutine_overlap.pdf}
    \caption{\textbf{Subprocess S6 for selecting overlap-based segmentation metrics (if any)}. Applies to: semantic segmentation (SemS) and instance segmentation (InS). Decision guides are provided in Suppl. Note~\ref{ssec:dg6}. A detailed description of the subprocess is given in Suppl. Notes~\ref{app:ss} and \ref{app:is}.}
    \label{fig:metric-selection:s6-overlap}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{images/MetricMappings/S7_subroutine_boundary.pdf}
    % \includegraphics[width=1\linewidth]{images/MetricMappings/Delta/S7_subroutine_boundary.pdf}
    \caption{\textbf{Subprocess S7 for selecting a boundary-based segmentation metric (if any)}. Applies to: semantic segmentation (SemS) and instance segmentation (InS). Decision guides are provided in Suppl. Note~\ref{ssec:dg7}. A detailed description of the subprocess is given in Suppl. Notes~\ref{app:ss} and \ref{app:is}.}
    \label{fig:metric-selection:s7-boundary}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{images/MetricMappings/S8_subroutine_localization.pdf}
    % \includegraphics[width=1\linewidth]{images/MetricMappings/Delta/S8_subroutine_localization.pdf}
    \caption{\textbf{Subprocess S8 for selecting the localization criterion}. Applies to: object detection (ObD) and instance segmentation (InS). Definitions of the localization criteria can be found in \cite{reinke2021common}. Decision guides are provided in Suppl. Note~\ref{ssec:dg8}. A detailed description of the subprocess is given in Suppl. Notes~\ref{app:od} and \ref{app:is}.}
    \label{fig:metric-selection:s8-localization-criterion}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{images/MetricMappings/S9_subroutine_assignment.pdf}
    % \includegraphics[width=1\linewidth]{images/MetricMappings/Delta/S9_subroutine_assignment.pdf}
    \caption{\textbf{Subprocess S9 for selecting the assignment strategy.} Applies to: object detection (ObD) and instance segmentation (InS). Assignment strategies are defined in \cite{reinke2021common}. Decision guides are provided in Suppl. Note~\ref{ssec:dg9}. A detailed description of the subprocess is given in Suppl. Notes~\ref{app:od} and \ref{app:is}.}
    \label{fig:metric-selection:s9-assignment-strategy}
\end{figure}


